Neurosymbolic Decision Trees

Neurosymbolic (NeSy) AI studies the integration of neural networks (NNs) and symbolic reasoning based on logic. Usually, NeSy techniques focus on learning the neural, probabilistic and/or fuzzy parameters of NeSy models. Learning the symbolic or logical structure of such models has, so far, received less attention. We introduce neurosymbolic decision trees (NDTs), as an extension of decision trees together with a novel NeSy structure learning algorithm, which we dub NeuID3. NeuID3 adapts the standard top-down induction of decision tree algorithms and combines it with a neural probabilistic logic representation, inherited from the DeepProbLog family of models. The key advantage of learning NDTs with NeuID3 is the support of both symbolic and subsymbolic data (such as images), and that they can exploit background knowledge during the induction of the tree structure, In our experimental evaluation we demonstrate the benefits of NeSys structure learning over more traditonal approaches such as purely data-driven learning with neural networks.

==> graphics/experiments/experiment_eleusis/detected_tests.tex <==
%\ifstandalone
%\documentclass{standalone}

%\usepackage{tikz, pgf}

%\standaloneenv{new_image}

%\begin{document}
%\fi

\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccc}
\toprule
rule & uses bgk & counts & \multicolumn{2}{c}{score ratio} \\
 &  & & mean & std \\
\midrule
\multirow[t]{2}{*}{alternating\_faces} & True & 25 & 0.83 & 0.14 \\
 & False & 3 & 1.16 & 0.23 \\
\cline{1-5}
\multirow[t]{2}{*}{alternating\_parity} & True & 26 & 0.85 & 0.16 \\
 & False & 2 & 1.02 & 0.03 \\
\cline{1-5}
\multirow[t]{2}{*}{color\_parity\_rule} &  True & 14 & 0.98 & 0.02 \\
 &False & 14 & 1.01 & 0.01 \\
\cline{1-5}
\multirow[t]{2}{*}{hidden\_modulo\_simple} & True & 6 & 0.60 & 0.21 \\
 & False & 31 & 1.60 & 0.35 \\
\cline{1-5}
\multirow[t]{2}{*}{hidden\_order\_simple} & True & 6 & 0.54 & 0.46 \\
 & False & 36 & 1.62 & 0.32 \\
\cline{1-5}
\multirow[t]{2}{*}{increase\_suits} & True & 22 & 0.95 & 0.09 \\
 & False & 6 & 1.01 & 0.01 \\
\cline{1-5}
\multirow[t]{2}{*}{rank\_order} & True & 19 & 0.96 & 0.04 \\
 & False & 9 & 1.01 & 0.01 \\
\cline{1-5}
\multirow[t]{2}{*}{suit\_order} & True & 19 & 0.98 & 0.02 \\
 & False & 9 & 1.01 & 0.01 \\
\cline{1-5}
\bottomrule
\end{tabular*}

%\ifstandalone
%\end{document}
%\fi


==> graphics/experiments/experiment_eleusis/results_without_neural_baseline.tex <==
\begin{tabular}{l|llll|llll}
\toprule
 & \multicolumn{4}{c|}{Number of Ranks=7} & \multicolumn{4}{c|}{Number of Ranks=8} \\
 & NDT(bad pool) & NDT(neural preds) & NDT(general pool) & NDT(optimal pool) & NDT(bad pool) & NDT(neural preds) & NDT(general pool) & NDT(optimal pool) \\
\midrule
\multicolumn{8}{l}{F1 score (Positives)}\\
\midrule
hidden\_modulo\_simple%
 & $0.773\pm0.103$ & $0.851\pm0.010$ & $0.852\pm0.017$ & $\mathbf{0.891}\pm0.015$%
 & $0.833\pm0.072$ & $0.876\pm0.014$ & $0.880\pm0.017$ & $\mathbf{0.905}\pm0.008$ \\
hidden\_order\_simple%
 & $0.733\pm0.025$ & $\mathbf{0.760}\pm0.029$ & $0.746\pm0.033$ & $0.753\pm0.029$%
 & $0.697\pm0.026$ & $0.695\pm0.035$ & $0.708\pm0.021$ & $\mathbf{0.748}\pm0.045$ \\
color\_parity\_rule%
 & $0.977\pm0.008$ & $0.977\pm0.005$ & $0.979\pm0.004$ & $\mathbf{0.986}\pm0.003$%
 & $0.968\pm0.008$ & $0.977\pm0.007$ & $0.980\pm0.006$ & $\mathbf{0.983}\pm0.003$ \\
increase\_suits%
 & $0.981\pm0.005$ & $0.983\pm0.004$ & $0.989\pm0.007$ & $\mathbf{0.990}\pm0.002$%
 & $0.969\pm0.024$ & $0.973\pm0.027$ & $0.991\pm0.004$ & $\mathbf{0.992}\pm0.003$ \\
suit\_order%
 & $0.980\pm0.006$ & $0.986\pm0.003$ & $0.991\pm0.007$ & $\mathbf{0.994}\pm0.003$%
 & $0.981\pm0.005$ & $0.985\pm0.004$ & $0.991\pm0.005$ & $\mathbf{0.993}\pm0.003$ \\
rank\_order%
 & $0.904\pm0.008$ & $0.918\pm0.013$ & $0.971\pm0.025$ & $\mathbf{0.977}\pm0.005$%
 & $0.857\pm0.011$ & $0.877\pm0.015$ & $0.956\pm0.031$ & $\mathbf{0.970}\pm0.006$ \\
alternating\_parity%
 & $0.906\pm0.016$ & $0.931\pm0.009$ & $0.974\pm0.006$ & $\mathbf{0.980}\pm0.003$%
 & $0.862\pm0.033$ & $0.871\pm0.057$ & $0.959\pm0.026$ & $\mathbf{0.977}\pm0.006$ \\
alternating\_faces%
 & $0.859\pm0.150$ & $0.899\pm0.067$ & $\mathbf{0.960}\pm0.014$ & $\mathbf{0.960}\pm0.017$%
 & $0.727\pm0.204$ & $0.740\pm0.194$ & $0.937\pm0.022$ & $\mathbf{0.948}\pm0.029$ \\
\midrule
\multicolumn{8}{l}{F1 score (Negatives)}\\
\midrule
hidden\_modulo\_simple%
 & $0.620\pm0.165$ & $0.733\pm0.008$ & $0.733\pm0.022$ & $\mathbf{0.763}\pm0.036$%
 & $0.687\pm0.121$ & $0.752\pm0.015$ & $0.758\pm0.026$ & $\mathbf{0.774}\pm0.026$ \\
hidden\_order\_simple%
 & $0.875\pm0.010$ & $\mathbf{0.887}\pm0.017$ & $0.874\pm0.012$ & $0.863\pm0.025$%
 & $0.850\pm0.012$ & $0.850\pm0.019$ & $0.858\pm0.014$ & $\mathbf{0.863}\pm0.024$ \\
color\_parity\_rule%
 & $0.978\pm0.008$ & $0.978\pm0.006$ & $0.980\pm0.004$ & $\mathbf{0.986}\pm0.004$%
 & $0.968\pm0.008$ & $0.976\pm0.007$ & $0.980\pm0.006$ & $\mathbf{0.982}\pm0.004$ \\
increase\_suits%
 & $0.943\pm0.015$ & $0.949\pm0.014$ & $0.968\pm0.019$ & $\mathbf{0.971}\pm0.007$%
 & $0.902\pm0.087$ & $0.917\pm0.090$ & $0.972\pm0.010$ & $\mathbf{0.976}\pm0.008$ \\
suit\_order%
 & $0.968\pm0.010$ & $0.977\pm0.005$ & $0.985\pm0.012$ & $\mathbf{0.991}\pm0.005$%
 & $0.971\pm0.008$ & $0.976\pm0.008$ & $0.986\pm0.009$ & $\mathbf{0.989}\pm0.003$ \\
rank\_order%
 & $0.881\pm0.014$ & $0.901\pm0.012$ & $0.963\pm0.031$ & $\mathbf{0.971}\pm0.007$%
 & $0.824\pm0.016$ & $0.844\pm0.020$ & $0.945\pm0.037$ & $\mathbf{0.963}\pm0.008$ \\
alternating\_parity%
 & $0.912\pm0.012$ & $0.935\pm0.009$ & $0.976\pm0.005$ & $\mathbf{0.982}\pm0.003$%
 & $0.871\pm0.030$ & $0.883\pm0.045$ & $0.963\pm0.023$ & $\mathbf{0.979}\pm0.005$ \\
alternating\_faces%
 & $0.858\pm0.165$ & $0.901\pm0.075$ & $\mathbf{0.962}\pm0.013$ & $\mathbf{0.962}\pm0.017$%
 & $0.760\pm0.179$ & $0.764\pm0.177$ & $0.942\pm0.020$ & $\mathbf{0.952}\pm0.026$ \\
\bottomrule
\end{tabular}


==> graphics/methods/latexmkrc <==
$pdf_mode = 4;
$postscript_mode = $dvi_mode = 0;

# For minted
&set_tex_cmds( '-shell-escape %O %S' );
#&set_tex_cmds( '-shell-escape %O '
#    . '\'\PassOptionsToPackage{outputdir={%Y}}{minted}\input{%S}\' %S'
#    );
$hash_calc_ignore_pattern{aux} = '^\\\\gdef\\\\minted@oldcachelist\{,'.
                                 '|^\s*default\.pygstyle,'.
                                 '|^\s*[[:xdigit:]]+\.pygtex';


==> latexmkrc <==
$pdf_mode = 4;
$postscript_mode = $dvi_mode = 0;

# For minted
&set_tex_cmds( '-shell-escape %O %S' );
#&set_tex_cmds( '-shell-escape %O '
#    . '\'\PassOptionsToPackage{outputdir={%Y}}{minted}\input{%S}\' %S'
#    );
$hash_calc_ignore_pattern{aux} = '^\\\\gdef\\\\minted@oldcachelist\{,'.
                                 '|^\s*default\.pygstyle,'.
                                 '|^\s*[[:xdigit:]]+\.pygtex';

